Learning to Solve the Constrained Most Probable Explanation Task in Probabilistic Graphical Models

We propose a self-supervised learning approach for solving the following constrained optimization task in log-linear models or Markov networks. Let $f$ and $g$ be two log-linear models defined over the sets $\mathbf{X}$ and $\mathbf{Y}$ of random variables respectively. Given an assignment $\mathbf{x}$ to all variables in $\mathbf{X}$ (evidence) and a real number $q$, the constrained most-probable explanation (CMPE) task seeks to find an assignment $\mathbf{y}$ to all variables in $\mathbf{Y}$ such that $f(\mathbf{x}, \mathbf{y})$ is maximized and $g(\mathbf{x}, \mathbf{y})\leq q$. In our proposed self-supervised approach, given assignments $\mathbf{x}$ to $\mathbf{X}$ (data), we train a deep neural network that learns to output near-optimal solutions to the CMPE problem without requiring access to any pre-computed solutions. The key idea in our approach is to use first principles and approximate inference methods for CMPE to derive novel loss functions that seek to push infeasible solutions towards feasible ones and feasible solutions towards optimal ones. We analyze the properties of our proposed method and experimentally demonstrate its efficacy on several benchmark problems.

==> content/figs/new_fig_1.tex <==
\begin{figure*}[htbp]  % Notice the asterisk in figure* for spanning two columns
    \centering
    \begin{subfigure}[b]{0.24\textwidth}  % Adjusted width to 0.24 for each subfigure
        \centering
        \includegraphics[width=\textwidth]{content/figs/aistats_fig_1.pdf}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \raisebox{15ex}{
        \begin{tabular}{|c|c|c|c|}
            \hline
             $X_1$ & $Y_1$ & $f_1$ & $g_1$   \\
             \hline
             0 & 0 & 4 & 10\\
             0 & 1 & 3 & 15\\
             1 & 0 & 1 & 12\\
             1 & 1 & 5 & 9\\
             \hline
        \end{tabular}
        }
        \caption{$f(x_1,y_1)=4-y_1-3x_1+8x_1y_1$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \raisebox{25ex}{
        \begin{tabular}{|c|c|c|c|}
            \hline
             $Y_1$ & $Y_2$ & $f_2$ & $g_2$   \\
             \hline
             0 & 0 & 7 & 1\\
             0 & 1 & 9 & 3\\
             1 & 0 & 3 & 2\\
             1 & 1 & 2 & 4\\
             \hline
        \end{tabular}
        }
        \caption{}
        
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \raisebox{25ex}{
        \begin{tabular}{|c|c|c|c|}
        \hline
         $X_2$ & $Y_2$ & $f_3$ & $g_3$   \\
         \hline
         0 & 0 & 3 & 17\\
         0 & 1 & 3 & 13\\
         1 & 0 & 8 & 10\\
         1 & 1 & 6 & 5\\
         \hline
        \end{tabular}
        }
        \caption{}
    \end{subfigure}
    \caption{\label{} Let $\mathcal{M}_1$ and $\mathcal{M}_2$ be two Markov networks defined over the set of variables $\mathbf{Z}=\{X_1,X_2,Y_1,Y_2\}$. $\mathcal{M}_1$ has the log potential functions $\{f_1(X_1,Y_1),f_2(Y_1,Y_@),f_3(X_2,Y_2)\}$ and $\mathcal{M}_2$ has the log-potential functions $\{g_1(X_1,Y_1),g_2(Y_1,Y_2),g_3(X_2,Y_2)\}$.  
\end{figure*}


==> content/mnist.tex <==
\begin{figure}
\small
    \centering
%\begin{table}[]
\begin{tabular}{lllllll}
\ilp:    & \includegraphics[scale=0.75]{content/figs/ilp-8.png}       & \includegraphics[scale=0.75]{content/figs/ilp-2.png}         & \includegraphics[scale=0.75]{content/figs/ilp-7.png}         & \includegraphics[scale=0.75]{content/figs/ilp-6.png}         & \multicolumn{2}{l}{\includegraphics[scale=0.75]{content/figs/ilp-1.png}}         \\
\slpen:     & \includegraphics[scale=0.75]{content/figs/penalty_mse-8.png} & \includegraphics[scale=0.75]{content/figs/penalty_mse-2.png} & \includegraphics[scale=0.75]{content/figs/penalty_mse-7.png} & \includegraphics[scale=0.75]{content/figs/penalty_mse-6.png} & \multicolumn{2}{l}{\includegraphics[scale=0.75]{content/figs/penalty_MSE-1.png}} \\
\sslpen:    & \includegraphics[scale=0.75]{content/figs/ssl_penalty-8.png} & \includegraphics[scale=0.75]{content/figs/ssl_penalty-2.png} & \includegraphics[scale=0.75]{content/figs/ssl_penalty-7.png} & \includegraphics[scale=0.75]{content/figs/ssl_penalty-6.png} & \multicolumn{2}{l}{\includegraphics[scale=0.75]{content/figs/ssl_penalty-1.png}} \\
\pdl:    & \includegraphics[scale=0.75]{content/figs/pdl-8.png}         & \includegraphics[scale=0.75]{content/figs/pdl-2.png}         & \includegraphics[scale=0.75]{content/figs/pdl-7.png}         & \includegraphics[scale=0.75]{content/figs/pdl-6.png}         & \multicolumn{2}{l}{\includegraphics[scale=0.75]{content/figs/pdl-1.png}}         \\
\ours: & \includegraphics[scale=0.75]{content/figs/ours-8.png}        & \includegraphics[scale=0.75]{content/figs/ours-2.png}        & \includegraphics[scale=0.75]{content/figs/ours-7.png}        & \includegraphics[scale=0.75]{content/figs/ours-6.png}        & \includegraphics[scale=0.75]{content/figs/ours-1.png}             &             
\end{tabular}
%\end{table}    
    \eat{ILP:  \includegraphics[scale=0.75]{content/figs/ilp-8.png}\includegraphics[scale=0.75]{content/figs/ilp-2.png}\includegraphics[scale=0.75]{content/figs/ilp-7.png}\includegraphics[scale=0.75]{content/figs/ilp-6.png}\includegraphics[scale=0.75]{content/figs/ilp-1.png}\\
    SL:   \includegraphics[scale=1]{content/figs/penalty_mse-8.png}\includegraphics[scale=0.75]{content/figs/penalty_mse-2.png}\includegraphics[scale=0.75]{content/figs/penalty_mse-7.png}\includegraphics[scale=0.75]{content/figs/penalty_mse-6.png}\includegraphics[scale=0.75]{content/figs/penalty_MSE-1.png}\\
    SSL:  \includegraphics[scale=1]{content/figs/ssl_penalty-8.png}\includegraphics[scale=0.75]{content/figs/ssl_penalty-2.png}\includegraphics[scale=0.75]{content/figs/ssl_penalty-7.png}\includegraphics[scale=0.75]{content/figs/ssl_penalty-6.png}\includegraphics[scale=0.75]{content/figs/ssl_penalty-1.png}\\
    PDL:  \includegraphics[scale=1]{content/figs/pdl-8.png}\includegraphics[scale=0.75]{content/figs/pdl-2.png}\includegraphics[scale=0.75]{content/figs/pdl-7.png}\includegraphics[scale=0.75]{content/figs/pdl-6.png}\includegraphics[scale=0.75]{content/figs/pdl-1.png}\\
    Ours: \includegraphics[scale=1]{content/figs/ours-8.png}\includegraphics[scale=0.75]{content/figs/ours-2.png}\includegraphics[scale=0.75]{content/figs/ours-7.png}\includegraphics[scale=0.75]{content/figs/ours-6.png}\includegraphics[scale=0.75]{content/figs/ours-1.png}
    }\eat{
    \includegraphics[scale=0.14]{figs/o-8.png}\includegraphics[scale=0.14]{figs/o-9.png}\\
    \includegraphics[scale=0.14]{figs/m1-0.png}\includegraphics[scale=0.14]{figs/m1-3.png}\includegraphics[scale=0.14]{figs/m1-4.png}\includegraphics[scale=0.14]{figs/m1-5.png}\includegraphics[scale=0.14]{figs/m1-8.png}\includegraphics[scale=0.14]{figs/m1-9.png}\\
    \includegraphics[scale=0.14]{figs/m2-0.png}\includegraphics[scale=0.14]{figs/m2-3.png}\includegraphics[scale=0.14]{figs/m2-4.png}\includegraphics[scale=0.14]{figs/m2-5.png}\includegraphics[scale=0.14]{figs/m2-8.png}\includegraphics[scale=0.14]{figs/m2-9.png}}
    \caption{\label{fig:mnist} \eat{Qualitative results on the MNIST dataset. Each row represents an original image followed by the updated images generated by different methods: \ilp, \msepen, \ssl, \pdl, and \sscmpe. Notably, all methods successfully flip the class of the image, showcasing their ability to generate modified images belonging to a different class. The distinct differences observed in the updated images highlight the unique approaches employed by each method to achieve the class flip.
    \eat{Qualitative results on MNIST. Row 1 shows the original test images. Row 2 shows the images changed using the univariate model \textit{so that the decision changes} from the original classification to any one of the other $9$ digits. Row 3 shows the images changed using the grid model.}}
    Qualitative results on the adversarially generated MNIST digits. Each row represents an original image followed by a corresponding image generated adversarially by different methods: \ilp, \msepen, \ssl, \pdl, and \ours.}    \end{figure}


==> content/mnist_new.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{lllll}
\multicolumn{1}{c}{\ilp} & \multicolumn{1}{c}{\slpen } & \multicolumn{1}{c}{\sslpen} & \multicolumn{1}{c}{\pdl} & \multicolumn{1}{c}{\sscmpe } \\

% ILP                                                 & \slpen                                                          & \sslpen                                                         & \pdl                                                 & \sscmpe                                            \\
\includegraphics[scale=0.60]{content/figs/ilp-8.png} & \includegraphics[scale=0.60]{content/figs/penalty_mse-8.png}   & \includegraphics[scale=0.60]{content/figs/ssl_penalty-8.png}   & \includegraphics[scale=0.60]{content/figs/pdl-8.png}   & \includegraphics[scale=0.60]{content/figs/ours-8.png}   \\
\includegraphics[scale=0.60]{content/figs/ilp-2.png} & \includegraphics[scale=0.60]{content/figs/penalty_mse-2.png} & \includegraphics[scale=0.60]{content/figs/ssl_penalty-2.png} & \includegraphics[scale=0.60]{content/figs/pdl-2.png} & \includegraphics[scale=0.60]{content/figs/ours-2.png} \\
\includegraphics[scale=0.60]{content/figs/ilp-7.png} & \includegraphics[scale=0.60]{content/figs/penalty_mse-7.png} & \includegraphics[scale=0.60]{content/figs/ssl_penalty-7.png} & \includegraphics[scale=0.60]{content/figs/pdl-7.png} & \includegraphics[scale=0.60]{content/figs/ours-7.png} \\
\eat{\includegraphics[scale=0.60]{content/figs/ilp-6.png} & \includegraphics[scale=0.60]{content/figs/penalty_mse-6.png} & \includegraphics[scale=0.60]{content/figs/ssl_penalty-6.png} & \includegraphics[scale=0.60]{content/figs/pdl-6.png} & \includegraphics[scale=0.60]{content/figs/ours-6.png} \\
\includegraphics[scale=0.60]{content/figs/ilp-0.60.png} & \includegraphics[scale=0.60]{content/figs/penalty_MSE-0.60.png} & \includegraphics[scale=0.60]{content/figs/ssl_penalty-0.60.png} & \includegraphics[scale=0.60]{content/figs/pdl-0.60.png} & \includegraphics[scale=0.60]{content/figs/ours-0.60.png}}
\end{tabular}
\caption{\label{fig:mnist}Qualitative results on the adversarially generated MNIST digits. From the left, each row contains the original image followed by a corresponding image generated adversarially by different methods: \ilp, \slpen, \sslpen, \pdl, and \ours.}
\end{figure}

==> content/reproducibility_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
% Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% \textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}


==> content/table_adversarial.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\begin{tabular}{|c|c|c|c|ccc|}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Objective} & \multirow{2}{*}{Gap} & \multirow{2}{*}{Violations} & \multicolumn{3}{c|}{Time in seconds}                                                                               \\ \cline{5-7} 
                        &                            &                      &                             & \multicolumn{1}{c|}{Training}                 & \multicolumn{1}{c|}{Test}                   & Data Generation      \\ \hline
ILP                     & 30.794                     & 0.000                & 0.000                       & \multicolumn{1}{c|}{NA}                       & \multicolumn{1}{c|}{57298.59}               & 0                    \\ \hline
MAE+penalty             & 86.527                     & 1.812                & 0.356                       & \multicolumn{1}{c|}{374.153}                  & \multicolumn{1}{c|}{0.003}                  & 57298.59             \\ \hline
MSE+penalty             & 63.670                     & 1.069                & 0.071                       & \multicolumn{1}{c|}{358.430}                  & \multicolumn{1}{c|}{0.003}                  & 57298.59             \\ \hline
SSL+penalty             & 76.316                     & 1.480                & 0.052                       & \multicolumn{1}{c|}{469.540}                  & \multicolumn{1}{c|}{0.003}                  & N/A                  \\ \hline
PDL                     & 66.400                     & 1.158                & 0.055                       & \multicolumn{1}{c|}{839.025}                  & \multicolumn{1}{c|}{0.003}                  & N/A                  \\ \hline
SS-CMPE (Max)           & 74.727                     & 1.429                & \textcolor{blue}{0.016}              & \multicolumn{1}{c|}{\multirow{3}{*}{520.149}} & \multicolumn{1}{c|}{\multirow{3}{*}{0.003}} & \multirow{3}{*}{N/A} \\ \cline{1-4}
SS-CMPE (Min)           & \textcolor{blue}{62.400}            & \textcolor{blue}{1.028}       & 0.021                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}                       &                      \\ \cline{1-4}
SS-CMPE (Average)       & 64.262                     & 1.089                & 0.027                       & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}                       &                      \\ \hline
\end{tabular}
\end{table}

==> content/table_tractable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\begin{tabular}{|cccccc|}
\hline
\multicolumn{1}{|c|}{dataset}                        & \multicolumn{1}{c|}{dna}           & \multicolumn{1}{c|}{c20ng}         & \multicolumn{1}{c|}{cwebkb}        & \multicolumn{1}{c|}{ad}            & bbc           \\ \hline
\multicolumn{1}{|c|}{\ilp Obj.}                      & \multicolumn{1}{c|}{221.119}       & \multicolumn{1}{c|}{921.702}       & \multicolumn{1}{c|}{824.493}       & \multicolumn{1}{c|}{2519.128}      & 871.5666802   \\ \hline
\multicolumn{6}{|c|}{Gap}                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \msepen}} & \multicolumn{1}{c|}{0.143 ± 0.113} & \multicolumn{1}{c|}{0.041 ± 0.031} & \multicolumn{1}{c|}{0.044 ± 0.035} & \multicolumn{1}{c|}{0.156 ± 0.057} & 0.036 ± 0.027 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \ssl}}    & \multicolumn{1}{c|}{0.142 ± 0.116} & \multicolumn{1}{c|}{0.045 ± 0.036} & \multicolumn{1}{c|}{0.058 ± 0.043} & \multicolumn{1}{c|}{0.159 ± 0.055} & 0.045 ± 0.033 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \pdl}}    & \multicolumn{1}{c|}{0.144 ± 0.117} & \multicolumn{1}{c|}{0.046 ± 0.035} & \multicolumn{1}{c|}{0.059 ± 0.043} & \multicolumn{1}{c|}{0.154 ± 0.055} & 0.051 ± 0.036 \\
\multicolumn{1}{|c|}{\ourmax}                        & \multicolumn{1}{c|}{0.138 ± 0.112} & \multicolumn{1}{c|}{0.046 ± 0.035} & \multicolumn{1}{c|}{0.057 ± 0.042} & \multicolumn{1}{c|}{0.139 ± 0.055} & 0.044 ± 0.032 \\
\multicolumn{1}{|c|}{\ourmin}                        & \multicolumn{1}{c|}{0.140 ± 0.112} & \multicolumn{1}{c|}{0.045 ± 0.035} & \multicolumn{1}{c|}{0.057 ± 0.043} & \multicolumn{1}{c|}{0.134 ± 0.054} & 0.043 ± 0.033 \\
\multicolumn{1}{|c|}{\ouravg}                        & \multicolumn{1}{c|}{0.142 ± 0.111} & \multicolumn{1}{c|}{0.045 ± 0.035} & \multicolumn{1}{c|}{0.058 ± 0.042} & \multicolumn{1}{c|}{0.138 ± 0.055} & 0.043 ± 0.032 \\ \hline
\multicolumn{6}{|c|}{Violations}                                                                                                                                                                                         \\ \hline
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \msepen}} & \multicolumn{1}{c|}{0.151 ± 0.358} & \multicolumn{1}{c|}{0.084 ± 0.277} & \multicolumn{1}{c|}{0.070 ± 0.254} & \multicolumn{1}{c|}{0.135 ± 0.341} & 0.237 ± 0.425 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \ssl}}    & \multicolumn{1}{c|}{0.014 ± 0.118} & \multicolumn{1}{c|}{0.005 ± 0.071} & \multicolumn{1}{c|}{0.025 ± 0.158} & \multicolumn{1}{c|}{0.008 ± 0.089} & 0.056 ± 0.230 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \pdl}}    & \multicolumn{1}{c|}{0.006 ± 0.077} & \multicolumn{1}{c|}{0.004 ± 0.059} & \multicolumn{1}{c|}{0.012 ± 0.109} & \multicolumn{1}{c|}{0.000 ± 0.000} & 0.025 ± 0.156 \\
\multicolumn{1}{|c|}{\ourmax}                        & \multicolumn{1}{c|}{0.007 ± 0.083} & \multicolumn{1}{c|}{0.005 ± 0.071} & \multicolumn{1}{c|}{0.017 ± 0.129} & \multicolumn{1}{c|}{0.008 ± 0.089} & 0.056 ± 0.230 \\
\multicolumn{1}{|c|}{\ourmin}                        & \multicolumn{1}{c|}{0.005 ± 0.071} & \multicolumn{1}{c|}{0.006 ± 0.077} & \multicolumn{1}{c|}{0.016 ± 0.126} & \multicolumn{1}{c|}{0.006 ± 0.077} & 0.056 ± 0.230 \\
\multicolumn{1}{|c|}{\ouravg}                        & \multicolumn{1}{c|}{0.009 ± 0.092} & \multicolumn{1}{c|}{0.005 ± 0.071} & \multicolumn{1}{c|}{0.018 ± 0.133} & \multicolumn{1}{c|}{0.006 ± 0.080} & 0.061 ± 0.239 \\ \hline
\end{tabular}
\end{table}

==> content/table_uai.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\begin{tabular}{|cccccc|}
\hline
\multicolumn{6}{|c|}{UAI   benchmarks}                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|c|}{Models}                         & \multicolumn{1}{c|}{Segment12}       & \multicolumn{1}{c|}{Segment14}     & \multicolumn{1}{c|}{Segment15}     & \multicolumn{1}{c|}{Grids17}       & Grids18       \\ \hline
\multicolumn{1}{|c|}{\ilp Obj.}                      & \multicolumn{1}{c|}{463.454}         & \multicolumn{1}{c|}{471.205}       & \multicolumn{1}{c|}{514.287}       & \multicolumn{1}{c|}{2879.469}      & 4160.196      \\ \hline
\multicolumn{6}{|c|}{Gap}                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \msepen}} & \multicolumn{1}{c|}{0.053 ±   0.043} & \multicolumn{1}{c|}{0.053 ± 0.043} & \multicolumn{1}{c|}{0.053 ± 0.041} & \multicolumn{1}{c|}{0.092 ± 0.070} & 0.082 ± 0.065 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \ssl}}    & \multicolumn{1}{c|}{0.051 ± 0.042}   & \multicolumn{1}{c|}{0.065 ± 0.048} & \multicolumn{1}{c|}{0.056 ± 0.044} & \multicolumn{1}{c|}{0.089 ± 0.055} & 0.104 ± 0.062 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \pdl}}    & \multicolumn{1}{c|}{0.063 ± 0.050}   & \multicolumn{1}{c|}{0.055 ± 0.042} & \multicolumn{1}{c|}{0.063 ± 0.049} & \multicolumn{1}{c|}{0.102 ± 0.059} & 0.092 ± 0.061 \\
\multicolumn{1}{|c|}{\ourmax}                        & \multicolumn{1}{c|}{0.050 ± 0.040}   & \multicolumn{1}{c|}{0.051 ± 0.039} & \multicolumn{1}{c|}{0.051 ± 0.040} & \multicolumn{1}{c|}{0.083 ± 0.055} & 0.069 ± 0.051 \\
\multicolumn{1}{|c|}{\ourmin}                        & \multicolumn{1}{c|}{0.050 ± 0.041}   & \multicolumn{1}{c|}{0.050 ± 0.039} & \multicolumn{1}{c|}{0.051 ± 0.039} & \multicolumn{1}{c|}{0.067 ± 0.049} & 0.077 ± 0.055 \\
\multicolumn{1}{|c|}{\ouravg}                        & \multicolumn{1}{c|}{0.050 ± 0.041}   & \multicolumn{1}{c|}{0.050 ± 0.038} & \multicolumn{1}{c|}{0.052 ± 0.041} & \multicolumn{1}{c|}{0.081 ± 0.054} & 0.087 ± 0.058 \\ \hline
\multicolumn{6}{|c|}{Violations}                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \msepen}} & \multicolumn{1}{c|}{0.238 ±   0.426} & \multicolumn{1}{c|}{0.248 ± 0.432} & \multicolumn{1}{c|}{0.153 ± 0.361} & \multicolumn{1}{c|}{0.054 ± 0.226} & 0.053 ± 0.224 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \ssl}}    & \multicolumn{1}{c|}{0.149 ± 0.357}   & \multicolumn{1}{c|}{0.127 ± 0.332} & \multicolumn{1}{c|}{0.086 ± 0.281} & \multicolumn{1}{c|}{0.004 ± 0.059} & 0.005 ± 0.071 \\
\multicolumn{1}{|c|}{{\color[HTML]{1D1C1D} \pdl}}    & \multicolumn{1}{c|}{0.073 ± 0.261}   & \multicolumn{1}{c|}{0.120 ± 0.326} & \multicolumn{1}{c|}{0.016 ± 0.126} & \multicolumn{1}{c|}{0.000 ± 0.000} & 0.001 ± 0.022 \\
\multicolumn{1}{|c|}{\ourmax}                        & \multicolumn{1}{c|}{0.224 ± 0.417}   & \multicolumn{1}{c|}{0.288 ± 0.453} & \multicolumn{1}{c|}{0.112 ± 0.315} & \multicolumn{1}{c|}{0.003 ± 0.055} & 0.001 ± 0.022 \\
\multicolumn{1}{|c|}{\ourmin}                        & \multicolumn{1}{c|}{0.224 ± 0.417}   & \multicolumn{1}{c|}{0.272 ± 0.445} & \multicolumn{1}{c|}{0.116 ± 0.320} & \multicolumn{1}{c|}{0.001 ± 0.032} & 0.001 ± 0.022 \\
\multicolumn{1}{|c|}{\ouravg}                        & \multicolumn{1}{c|}{0.224 ± 0.417}   & \multicolumn{1}{c|}{0.273 ± 0.445} & \multicolumn{1}{c|}{0.091 ± 0.288} & \multicolumn{1}{c|}{0.072 ± 0.259} & 0.003 ± 0.055 \\ \hline
\end{tabular}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

